F-theory and M-theory perspectives on N=2 supersymmetric gauge theories in four dimensions

Deformations of the original F-theory background are proposed. These lead to multiple new dualities and physical phenomena. We concentrate on one model where we let seven-branes wrap a multi-centered Taub-NUT space instead of R4. This configuration provides a successful F-theory embedding of a class of recently proposed four-dimensional N = 2 superconformal (SCFT) \`a la Gaiotto. Aspects of Argyres- Seiberg duality, of the new Gaiotto duality, as well as of the branes network of Benini- Benvenuti and Tachikawa are captured by our construction. The supergravity theory for the conformal case is also briefly discussed. Extending our construction to the non-conformal case, we find interesting cascading behavior in four-dimensional gauge theories with N = 2 supersymmetry. Since the analysis of this unexpected phenomenon is quite difficult in the language of type IIB/F-theory, we turn to the type IIA/M-theory description where the origin of the N = 2 cascade is clarified. Using the T-dual type IIA brane language, we first start by studying the N = 1 supersymmetric cascading gauge theory found in type IIB string theory on p regular and M fractional D3-branes at the tip of the conifold. We reproduce the supersymmetric vacuum structure of this theory. We also show that the IIA analog of the non-supersymmetric state found by Kachru, Pearson and Verlinde in the IIB description is metastable in string theory, but the barrier for tunneling to the supersymmetric vacuum goes to infinity in the field theory limit. We then use the techniques we have developed to analyze the N = 2 supersymmetric gauge theory corresponding to regular and fractional D3-branes on a near-singular K3, and clarify the origin of the cascade in this theory.

==> bibSW.tex <==
\providecommand{\href}[2]{#2}\begingroup\raggedright\begin{thebibliography}{10%
0}

\bibitem{sw1}
N.~Seiberg and E.~Witten, {\it {Monopole Condensation, And Confinement In N=2
  Supersymmetric Yang-Mills Theory}},  {\em Nucl. Phys.} {\bf B426} (1994)
  19--52, [\href{http://xxx.lanl.gov/abs/hep-th/9407087}{{\tt
  hep-th/9407087}}].

\bibitem{sw2}
N.~Seiberg and E.~Witten, {\it {Monopoles, duality and chiral symmetry breaking
  in N=2 supersymmetric QCD}},  {\em Nucl. Phys.} {\bf B431} (1994) 484--550,
  [\href{http://xxx.lanl.gov/abs/hep-th/9408099}{{\tt hep-th/9408099}}].

\bibitem{BilalReview}
A.~Bilal, {\it {Duality in N=2 SUSY SU(2) Yang-Mills theory: A Pedagogical
  introduction to the work of Seiberg and Witten}},
  \href{http://xxx.lanl.gov/abs/hep-th/9601007}{{\tt hep-th/9601007}}.

\bibitem{LercheReview}
W.~Lerche, {\it {Introduction to Seiberg-Witten theory and its stringy
  origin}},  {\em Nucl. Phys. Proc. Suppl.} {\bf 55B} (1997) 83--117,
  [\href{http://xxx.lanl.gov/abs/hep-th/9611190}{{\tt hep-th/9611190}}].

\bibitem{ArgyresShapere}
P.~C. Argyres and A.~D. Shapere, {\it {The Vacuum Structure of N=2 SuperQCD
  with Classical Gauge Groups}},  {\em Nucl. Phys.} {\bf B461} (1996) 437--459,
  [\href{http://xxx.lanl.gov/abs/hep-th/9509175}{{\tt hep-th/9509175}}].

\bibitem{dougschwa}
M.~R. Douglas, D.~A. Lowe, and J.~H. Schwarz, {\it {Probing F-theory with
  multiple branes}},  {\em Phys. Lett.} {\bf B394} (1997) 297--301,
  [\href{http://xxx.lanl.gov/abs/hep-th/9612062}{{\tt hep-th/9612062}}].

\bibitem{KLYTsimpleADE}
A.~Klemm, W.~Lerche, S.~Yankielowicz, and S.~Theisen, {\it {Simple
  singularities and N=2 supersymmetric Yang-Mills theory}},  {\em Phys. Lett.}
  {\bf B344} (1995) 169--175,
  [\href{http://xxx.lanl.gov/abs/hep-th/9411048}{{\tt hep-th/9411048}}].

\bibitem{senF}
A.~Sen, {\it {F-theory and Orientifolds}},  {\em Nucl. Phys.} {\bf B475} (1996)
  562--578, [\href{http://xxx.lanl.gov/abs/hep-th/9605150}{{\tt
  hep-th/9605150}}].

\bibitem{bds}
T.~Banks, M.~R. Douglas, and N.~Seiberg, {\it {Probing F-theory with branes}},
  {\em Phys. Lett.} {\bf B387} (1996) 278--281,
  [\href{http://xxx.lanl.gov/abs/hep-th/9605199}{{\tt hep-th/9605199}}].

\bibitem{vafaF}
C.~Vafa, {\it {Evidence for F-Theory}},  {\em Nucl. Phys.} {\bf B469} (1996)
  403--418, [\href{http://xxx.lanl.gov/abs/hep-th/9602022}{{\tt
  hep-th/9602022}}].

\bibitem{Billo:2010mg}
M.~Billo, L.~Gallot, A.~Lerda, and I.~Pesando, {\it {F-theoretic versus
  microscopic description of a conformal N=2 SYM theory}},  {\em JHEP} {\bf
  1011} (2010) 041, [\href{http://xxx.lanl.gov/abs/1008.5240}{{\tt
  arXiv:1008.5240}}].

\bibitem{Billo:2011uc}
M.~Billo, M.~Frau, L.~Giacone, and A.~Lerda, {\it {Holographic non-perturbative
  corrections to gauge couplings}},  {\em JHEP} {\bf 1108} (2011) 007,
  [\href{http://xxx.lanl.gov/abs/1105.1869}{{\tt arXiv:1105.1869}}]. *
  Temporary entry *.

\bibitem{Billo':2011pr}
M.~Billo', M.~Frau, L.~Gallot, and A.~Lerda, {\it {The exact 8d chiral ring
  from 4d recursion relations}},  {\em JHEP} {\bf 1111} (2011) 077,
  [\href{http://xxx.lanl.gov/abs/1107.3691}{{\tt arXiv:1107.3691}}]. *
  Temporary entry *.

\bibitem{Nekrasov}
N.~A. Nekrasov, {\it {Seiberg-Witten Prepotential From Instanton Counting}},
  {\em Adv. Theor. Math. Phys.} {\bf 7} (2004) 831--864,
  [\href{http://xxx.lanl.gov/abs/hep-th/0206161}{{\tt hep-th/0206161}}].

\bibitem{AGT}
L.~F. Alday, D.~Gaiotto, and Y.~Tachikawa, {\it {Liouville Correlation
  Functions from Four-dimensional Gauge Theories}},  {\em Lett.Math.Phys.} {\bf
  91} (2010) 167--197, [\href{http://xxx.lanl.gov/abs/0906.3219}{{\tt
  arXiv:0906.3219}}].

\bibitem{gaiotto}
D.~Gaiotto, {\it {N=2 dualities}},
  \href{http://xxx.lanl.gov/abs/0904.2715}{{\tt arXiv:0904.2715}}.

\bibitem{DDG}
D.-E. Diaconescu, M.~R. Douglas, and J.~Gomis, {\it {Fractional branes and
  wrapped branes}},  {\em JHEP} {\bf 9802} (1998) 013,
  [\href{http://xxx.lanl.gov/abs/hep-th/9712230}{{\tt hep-th/9712230}}].

\bibitem{mukdas}
K.~Dasgupta and S.~Mukhi, {\it {Brane constructions, fractional branes and
  Anti-de Sitter domain walls}},  {\em JHEP} {\bf 9907} (1999) 008,
  [\href{http://xxx.lanl.gov/abs/hep-th/9904131}{{\tt hep-th/9904131}}].

\bibitem{poln2}
J.~Polchinski, {\it {N=2 Gauge / gravity duals}},  {\em Int.J.Mod.Phys.} {\bf
  A16} (2001) 707--718, [\href{http://xxx.lanl.gov/abs/hep-th/0011193}{{\tt
  hep-th/0011193}}].

\bibitem{bbt}
F.~Benini, S.~Benvenuti, and Y.~Tachikawa, {\it {Webs of five-branes and N=2
  superconformal field theories}},  {\em JHEP} {\bf 09} (2009) 052,
  [\href{http://xxx.lanl.gov/abs/0906.0359}{{\tt arXiv:0906.0359}}].

\bibitem{becker}
K.~Becker and M.~Becker, {\it {M theory on eight manifolds}},  {\em Nucl.Phys.}
  {\bf B477} (1996) 155--167,
  [\href{http://xxx.lanl.gov/abs/hep-th/9605053}{{\tt hep-th/9605053}}].

\bibitem{SVW}
S.~Sethi, C.~Vafa, and E.~Witten, {\it {Constraints on low-dimensional string
  compactifications}},  {\em Nucl. Phys.} {\bf B480} (1996) 213--224,
  [\href{http://xxx.lanl.gov/abs/hep-th/9606122}{{\tt hep-th/9606122}}].

\bibitem{DRS}
K.~Dasgupta, G.~Rajesh, and S.~Sethi, {\it {M theory, orientifolds and
  G-flux}},  {\em JHEP} {\bf 08} (1999) 023,
  [\href{http://xxx.lanl.gov/abs/hep-th/9908088}{{\tt hep-th/9908088}}].

\bibitem{gimpol}
E.~G. Gimon and J.~Polchinski, {\it {Consistency conditions for orientifolds
  and d manifolds}},  {\em Phys.Rev.} {\bf D54} (1996) 1667--1676,
  [\href{http://xxx.lanl.gov/abs/hep-th/9601038}{{\tt hep-th/9601038}}].

\bibitem{dhoker}
E.~D'Hoker, I.~M. Krichever, and D.~H. Phong, {\it {The effective prepotential
  of N = 2 supersymmetric SO(N(c)) and Sp(N(c)) gauge theories}},  {\em Nucl.
  Phys.} {\bf B489} (1997) 211--222,
  [\href{http://xxx.lanl.gov/abs/hep-th/9609145}{{\tt hep-th/9609145}}].

\bibitem{AMP}
P.~C. Argyres, R.~Maimon, and S.~Pelland, {\it {The M theory lift of two 06-
  planes and four D6-branes}},  {\em JHEP} {\bf 0205} (2002) 008,
  [\href{http://xxx.lanl.gov/abs/hep-th/0204127}{{\tt hep-th/0204127}}].

\bibitem{SeoUPenn}
J.~Seo, {\it {Singularity structure and massless dyons of pure Seiberg-Witten
  theories with SU and Sp gauge groups (Strings-Math 2011 proceedings to
  appear)}}, .

\bibitem{GST}
D.~Gaiotto, N.~Seiberg, and Y.~Tachikawa, {\it {Comments on scaling limits of
  4d N=2 theories}},  {\em JHEP} {\bf 01} (2011) 078,
  [\href{http://xxx.lanl.gov/abs/1011.4568}{{\tt arXiv:1011.4568}}].

\bibitem{EHIY}
T.~Eguchi, K.~Hori, K.~Ito, and S.-K. Yang, {\it {Study of $N=2$ Superconformal
  Field Theories in $4$ Dimensions}},  {\em Nucl. Phys.} {\bf B471} (1996)
  430--444, [\href{http://xxx.lanl.gov/abs/hep-th/9603002}{{\tt
  hep-th/9603002}}].

\bibitem{EH}
T.~Eguchi and K.~Hori, {\it {N=2 superconformal field theories in
  four-dimensions and A-D-E classification}},
  \href{http://xxx.lanl.gov/abs/hep-th/9607125}{{\tt hep-th/9607125}}.

\bibitem{SeoDasgupta}
J.~Seo and K.~Dasgupta, {\it {Singularity structure and massless dyons of pure
  ${\cal N} = 2$ theories with $SU(r+1)$ and $Sp(2r)$ gauge groups}},  {\em To
  appear} (2011).

\bibitem{ArgyresDouglas}
P.~C. Argyres and M.~R. Douglas, {\it {New phenomena in SU(3) supersymmetric
  gauge theory}},  {\em Nucl.Phys.} {\bf B448} (1995) 93--126,
  [\href{http://xxx.lanl.gov/abs/hep-th/9505062}{{\tt hep-th/9505062}}].

\bibitem{ADJMwall}
E.~Andriyash, F.~Denef, D.~L. Jafferis, and G.~W. Moore, {\it {Bound state
  transformation walls}},  \href{http://xxx.lanl.gov/abs/1008.3555}{{\tt
  arXiv:1008.3555}}.

\bibitem{Seo}
J.~Seo, {\it {Scaling behaviour at maximal Argyres-Douglas points of pure
  $SO(2r+1)$ and $Sp(2r)$ Seiberg-Witten theory (work in progress)}}, .

\bibitem{FS}
A.~Fayyazuddin and M.~Spalinski, {\it {Large N superconformal gauge theories
  and supergravity orientifolds}},  {\em Nucl.Phys.} {\bf B535} (1998)
  219--232, [\href{http://xxx.lanl.gov/abs/hep-th/9805096}{{\tt
  hep-th/9805096}}].

\bibitem{DM1}
K.~Dasgupta and S.~Mukhi, {\it {F theory at constant coupling}},  {\em
  Phys.Lett.} {\bf B385} (1996) 125--131,
  [\href{http://xxx.lanl.gov/abs/hep-th/9606044}{{\tt hep-th/9606044}}].

\bibitem{AFM}
O.~Aharony, A.~Fayyazuddin, and J.~M. Maldacena, {\it {The Large N limit of
  N=2, N=1 field theories from three-branes in F theory}},  {\em JHEP} {\bf
  9807} (1998) 013, [\href{http://xxx.lanl.gov/abs/hep-th/9806159}{{\tt
  hep-th/9806159}}].

\bibitem{wittenTN}
E.~Witten, {\it {Branes, Instantons, And Taub-NUT Spaces}},  {\em JHEP} {\bf
  0906} (2009) 067, [\href{http://xxx.lanl.gov/abs/0902.0948}{{\tt
  arXiv:0902.0948}}].

\bibitem{aspinwall}
P.~S. Aspinwall, {\it {Enhanced gauge symmetries and K3 surfaces}},  {\em
  Phys.Lett.} {\bf B357} (1995) 329--334,
  [\href{http://xxx.lanl.gov/abs/hep-th/9507012}{{\tt hep-th/9507012}}].

\bibitem{poln3}
M.~Grana and J.~Polchinski, {\it {Gauge / gravity duals with holomorphic
  dilaton}},  {\em Phys.Rev.} {\bf D65} (2002) 126005,
  [\href{http://xxx.lanl.gov/abs/hep-th/0106014}{{\tt hep-th/0106014}}].

\bibitem{aharonyn2}
O.~Aharony, {\it {A Note on the holographic interpretation of string theory
  backgrounds with varying flux}},  {\em JHEP} {\bf 0103} (2001) 012,
  [\href{http://xxx.lanl.gov/abs/hep-th/0101013}{{\tt hep-th/0101013}}].

\bibitem{BDGreen}
C.~P. Bachas, M.~R. Douglas, and M.~B. Green, {\it {Anomalous creation of
  branes}},  {\em JHEP} {\bf 9707} (1997) 002,
  [\href{http://xxx.lanl.gov/abs/hep-th/9705074}{{\tt hep-th/9705074}}].

\bibitem{callan}
C.~G. Callan and J.~M. Maldacena, {\it {Brane dynamics from the Born-Infeld
  action}},  {\em Nucl. Phys.} {\bf B513} (1998) 198--212,
  [\href{http://xxx.lanl.gov/abs/hep-th/9708147}{{\tt hep-th/9708147}}].

\bibitem{wittenM}
E.~Witten, {\it {Solutions of four-dimensional field theories via M- theory}},
  {\em Nucl. Phys.} {\bf B500} (1997) 3--42,
  [\href{http://xxx.lanl.gov/abs/hep-th/9703166}{{\tt hep-th/9703166}}].

\bibitem{GM}
D.~Gaiotto and J.~Maldacena, {\it {The gravity duals of N=2 superconformal
  field theories}},  \href{http://xxx.lanl.gov/abs/0904.4466}{{\tt
  arXiv:0904.4466}}.

\bibitem{townsend1}
D.~Mateos and P.~K. Townsend, {\it {Supertubes}},  {\em Phys.Rev.Lett.} {\bf
  87} (2001) 011602, [\href{http://xxx.lanl.gov/abs/hep-th/0103030}{{\tt
  hep-th/0103030}}].

\bibitem{townsend2}
R.~Emparan, D.~Mateos, and P.~K. Townsend, {\it {Supergravity supertubes}},
  {\em JHEP} {\bf 0107} (2001) 011,
  [\href{http://xxx.lanl.gov/abs/hep-th/0106012}{{\tt hep-th/0106012}}].

\bibitem{bk}
D.-s. Bak and A.~Karch, {\it {Supersymmetric brane-antibrane configurations}},
  {\em Nucl. Phys.} {\bf B626} (2002) 165--182,
  [\href{http://xxx.lanl.gov/abs/hep-th/0110039}{{\tt hep-th/0110039}}].

\bibitem{gsvy}
B.~R. Greene, A.~D. Shapere, C.~Vafa, and S.-T. Yau, {\it {Stringy Cosmic
  Strings and Noncompact Calabi-Yau Manifolds}},  {\em Nucl.Phys.} {\bf B337}
  (1990) 1.

\bibitem{ghm}
R.~Gregory, J.~A. Harvey, and G.~W. Moore, {\it {Unwinding strings and t
  duality of Kaluza-Klein and h monopoles}},  {\em Adv.Theor.Math.Phys.} {\bf
  1} (1997) 283--297, [\href{http://xxx.lanl.gov/abs/hep-th/9708086}{{\tt
  hep-th/9708086}}].

\bibitem{tong}
D.~Tong, {\it {NS5-branes, T duality and world sheet instantons}},  {\em JHEP}
  {\bf 0207} (2002) 013, [\href{http://xxx.lanl.gov/abs/hep-th/0204186}{{\tt
  hep-th/0204186}}].

\bibitem{kleban}
M.~Kleban and M.~Redi, {\it {Expanding F-Theory}},  {\em JHEP} {\bf 0709}
  (2007) 038, [\href{http://xxx.lanl.gov/abs/0705.2020}{{\tt
  arXiv:0705.2020}}].

\bibitem{dhhk}
K.~Dasgupta, C.~Herdeiro, S.~Hirano, and R.~Kallosh, {\it {D3/D7 inflationary
  model and M-theory}},  {\em Phys. Rev.} {\bf D65} (2002) 126002,
  [\href{http://xxx.lanl.gov/abs/hep-th/0203019}{{\tt hep-th/0203019}}].

\bibitem{tate}
J.~Tate, {\it {Algorithm for determining the type of a singular fibre in an
  elliptic pencil}},  {\em {\it Modular functions of one variable IV}, Lecture
  notes in math. Springer-Verlag, Berlin} {\bf 476} (1975).

\bibitem{bikmsv}
M.~Bershadsky, K.~A. Intriligator, S.~Kachru, D.~R. Morrison, V.~Sadov, {\em
  et.~al.}, {\it {Geometric singularities and enhanced gauge symmetries}},
  {\em Nucl.Phys.} {\bf B481} (1996) 215--252,
  [\href{http://xxx.lanl.gov/abs/hep-th/9605200}{{\tt hep-th/9605200}}].

\bibitem{DMstring}
K.~Dasgupta and S.~Mukhi, {\it {BPS nature of three string junctions}},  {\em
  Phys.Lett.} {\bf B423} (1998) 261--264,
  [\href{http://xxx.lanl.gov/abs/hep-th/9711094}{{\tt hep-th/9711094}}].

\bibitem{minahan1}
J.~A. Minahan and D.~Nemeschansky, {\it {An N=2 superconformal fixed point with
  E(6) global symmetry}},  {\em Nucl.Phys.} {\bf B482} (1996) 142--152,
  [\href{http://xxx.lanl.gov/abs/hep-th/9608047}{{\tt hep-th/9608047}}].

\bibitem{minahan2}
J.~A. Minahan and D.~Nemeschansky, {\it {Superconformal fixed points with E(n)
  global symmetry}},  {\em Nucl.Phys.} {\bf B489} (1997) 24--46,
  [\href{http://xxx.lanl.gov/abs/hep-th/9610076}{{\tt hep-th/9610076}}].

\bibitem{sa}
P.~C. Argyres and N.~Seiberg, {\it {S-duality in N=2 supersymmetric gauge
  theories}},  {\em JHEP} {\bf 12} (2007) 088,
  [\href{http://xxx.lanl.gov/abs/0711.0054}{{\tt arXiv:0711.0054}}].

\bibitem{gaberdiel}
M.~R. Gaberdiel and B.~Zwiebach, {\it {Exceptional groups from open strings}},
  {\em Nucl. Phys.} {\bf B518} (1998) 151--172,
  [\href{http://xxx.lanl.gov/abs/hep-th/9709013}{{\tt hep-th/9709013}}].

\bibitem{benini2}
R.~Argurio, F.~Benini, M.~Bertolini, C.~Closset, and S.~Cremonesi, {\it
  {Gauge/gravity duality and the interplay of various fractional branes}},
  {\em Phys.Rev.} {\bf D78} (2008) 046008,
  [\href{http://xxx.lanl.gov/abs/0804.4470}{{\tt arXiv:0804.4470}}].

\bibitem{benini3}
F.~Benini, M.~Bertolini, C.~Closset, and S.~Cremonesi, {\it {The N=2 cascade
  revisited and the enhancon bearings}},  {\em Phys.Rev.} {\bf D79} (2009)
  066012, [\href{http://xxx.lanl.gov/abs/0811.2207}{{\tt arXiv:0811.2207}}].

\bibitem{ouyang1}
P.~Ouyang, {\it {Holomorphic D7 branes and flavored N=1 gauge theories}},  {\em
  Nucl.Phys.} {\bf B699} (2004) 207--225,
  [\href{http://xxx.lanl.gov/abs/hep-th/0311084}{{\tt hep-th/0311084}}].

\bibitem{ouyang2}
H.-Y. Chen, P.~Ouyang, and G.~Shiu, {\it {On Supersymmetric D7-branes in the
  Warped Deformed Conifold}},  {\em JHEP} {\bf 1001} (2010) 028,
  [\href{http://xxx.lanl.gov/abs/0807.2428}{{\tt arXiv:0807.2428}}]. *
  Temporary entry *.

\bibitem{KSks}
I.~R. Klebanov and M.~J. Strassler, {\it {Supergravity and a confining gauge
  theory: Duality cascades and chi SB resolution of naked singularities}},
  {\em JHEP} {\bf 0008} (2000) 052,
  [\href{http://xxx.lanl.gov/abs/hep-th/0007191}{{\tt hep-th/0007191}}].

\bibitem{neksav}
A.~Mikhailov, N.~Nekrasov, and S.~Sethi, {\it {Geometric realizations of BPS
  states in N=2 theories}},  {\em Nucl.Phys.} {\bf B531} (1998) 345--362,
  [\href{http://xxx.lanl.gov/abs/hep-th/9803142}{{\tt hep-th/9803142}}].

\bibitem{becker4}
K.~Becker, M.~Becker, P.~S. Green, K.~Dasgupta, and E.~Sharpe, {\it
  {Compactifications of heterotic strings on nonKahler complex manifolds. 2.}},
   {\em Nucl.Phys.} {\bf B678} (2004) 19--100,
  [\href{http://xxx.lanl.gov/abs/hep-th/0310058}{{\tt hep-th/0310058}}].

\bibitem{strominger}
B.~R. Greene, D.~R. Morrison, and A.~Strominger, {\it {Black hole condensation
  and the unification of string vacua}},  {\em Nucl.Phys.} {\bf B451} (1995)
  109--120, [\href{http://xxx.lanl.gov/abs/hep-th/9504145}{{\tt
  hep-th/9504145}}].

\bibitem{stromtor}
A.~Strominger, {\it {Superstrings with Torsion}},  {\em Nucl.Phys.} {\bf B274}
  (1986) 253.

\bibitem{carluest}
G.~Lopes~Cardoso, G.~Curio, G.~Dall'Agata, D.~Lust, P.~Manousselis, {\em
  et.~al.}, {\it {NonKahler string backgrounds and their five torsion
  classes}},  {\em Nucl.Phys.} {\bf B652} (2003) 5--34,
  [\href{http://xxx.lanl.gov/abs/hep-th/0211118}{{\tt hep-th/0211118}}].

\bibitem{becker1}
K.~Becker and K.~Dasgupta, {\it {Heterotic strings with torsion}},  {\em JHEP}
  {\bf 0211} (2002) 006, [\href{http://xxx.lanl.gov/abs/hep-th/0209077}{{\tt
  hep-th/0209077}}].

\bibitem{becker2}
K.~Becker, M.~Becker, K.~Dasgupta, and P.~S. Green, {\it {Compactifications of
  heterotic theory on nonKahler complex manifolds. 1.}},  {\em JHEP} {\bf 0304}
  (2003) 007, [\href{http://xxx.lanl.gov/abs/hep-th/0301161}{{\tt
  hep-th/0301161}}].

\bibitem{becker3}
K.~Becker, M.~Becker, K.~Dasgupta, and S.~Prokushkin, {\it {Properties of
  heterotic vacua from superpotentials}},  {\em Nucl.Phys.} {\bf B666} (2003)
  144--174, [\href{http://xxx.lanl.gov/abs/hep-th/0304001}{{\tt
  hep-th/0304001}}].

\bibitem{chen1}
F.~Chen, K.~Dasgupta, P.~Franche, S.~Katz, and R.~Tatar, {\it {Supersymmetric
  Configurations, Geometric Transitions and New Non-Kahler Manifolds}},  {\em
  Nucl.Phys.} {\bf B852} (2011) 553--591,
  [\href{http://xxx.lanl.gov/abs/1007.5316}{{\tt arXiv:1007.5316}}].

\bibitem{chen2}
F.~Chen, K.~Dasgupta, P.~Franche, and R.~Tatar, {\it {Toward the Gravity Dual
  of Heterotic Small Instantons}},  {\em Phys.Rev.} {\bf D83} (2011) 046006,
  [\href{http://xxx.lanl.gov/abs/1010.5509}{{\tt arXiv:1010.5509}}].

\bibitem{gauntlett}
J.~P. Gauntlett, D.~Martelli, and D.~Waldram, {\it {Superstrings with intrinsic
  torsion}},  {\em Phys. Rev.} {\bf D69} (2004) 086002,
  [\href{http://xxx.lanl.gov/abs/hep-th/0302158}{{\tt hep-th/0302158}}].

\bibitem{papado}
J.~Gutowski, S.~Ivanov, and G.~Papadopoulos, {\it {Deformations of generalized
  calibrations and compact nonKahler manifolds with vanishing first Chern
  class}},  \href{http://xxx.lanl.gov/abs/math/0205012}{{\tt math/0205012}}.

\bibitem{sav}
K.~Dasgupta, G.~Rajesh, D.~Robbins, and S.~Sethi, {\it {Time-dependent warping,
  fluxes, and NCYM}},  {\em JHEP} {\bf 03} (2003) 041,
  [\href{http://xxx.lanl.gov/abs/hep-th/0302049}{{\tt hep-th/0302049}}].

\bibitem{louisL}
S.~Gurrieri, J.~Louis, A.~Micu, and D.~Waldram, {\it {Mirror symmetry in
  generalized Calabi-Yau compactifications}},  {\em Nucl.Phys.} {\bf B654}
  (2003) 61--113, [\href{http://xxx.lanl.gov/abs/hep-th/0211102}{{\tt
  hep-th/0211102}}].

\bibitem{vafaBA}
C.~Vafa, {\it {Brane / anti-brane systems and $U(N\vert M)$ supergroup}},
  \href{http://xxx.lanl.gov/abs/hep-th/0101218}{{\tt hep-th/0101218}}.

\bibitem{ABSV08}
M.~Aganagic, C.~Beem, J.~Seo, and C.~Vafa, {\it {Extended Supersymmetric Moduli
  Space and a SUSY/Non-SUSY Duality}},  {\em Nucl. Phys.} {\bf B822} (2009)
  135--171, [\href{http://xxx.lanl.gov/abs/0804.2489}{{\tt arXiv:0804.2489}}].

\bibitem{superd}
E.~Bergshoeff and P.~Townsend, {\it {Super D-branes}},  {\em Nucl.Phys.} {\bf
  B490} (1997) 145--162, [\href{http://xxx.lanl.gov/abs/hep-th/9611173}{{\tt
  hep-th/9611173}}].

\bibitem{senstring}
A.~Sen, {\it {String network}},  {\em JHEP} {\bf 9803} (1998) 005,
  [\href{http://xxx.lanl.gov/abs/hep-th/9711130}{{\tt hep-th/9711130}}].

\bibitem{DMM}
K.~Dasgupta and S.~Mukhi, {\it {A Note on low dimensional string
  compactifications}},  {\em Phys.Lett.} {\bf B398} (1997) 285--290,
  [\href{http://xxx.lanl.gov/abs/hep-th/9612188}{{\tt hep-th/9612188}}].

\bibitem{GVW}
S.~Gukov, C.~Vafa, and E.~Witten, {\it {CFT's from Calabi-Yau four folds}},
  {\em Nucl.Phys.} {\bf B584} (2000) 69--108,
  [\href{http://xxx.lanl.gov/abs/hep-th/9906070}{{\tt hep-th/9906070}}].

\bibitem{BFSS}
T.~Banks, W.~Fischler, S.~Shenker, and L.~Susskind, {\it {M theory as a matrix
  model: A Conjecture}},  {\em Phys.Rev.} {\bf D55} (1997) 5112--5128,
  [\href{http://xxx.lanl.gov/abs/hep-th/9610043}{{\tt hep-th/9610043}}].

\bibitem{quivers}
M.~R. Douglas and G.~W. Moore, {\it {D-branes, quivers, and ALE instantons}},
  \href{http://xxx.lanl.gov/abs/hep-th/9603167}{{\tt hep-th/9603167}}.

\bibitem{DOS}
M.~R. Douglas, H.~Ooguri, and S.~H. Shenker, {\it {Issues in (M)atrix model
  compactification}},  {\em Phys.Lett.} {\bf B402} (1997) 36--42,
  [\href{http://xxx.lanl.gov/abs/hep-th/9702203}{{\tt hep-th/9702203}}].

\bibitem{raja}
W.~Fischler and A.~Rajaraman, {\it {M(atrix) string theory on K3}},  {\em
  Phys.Lett.} {\bf B411} (1997) 53--58,
  [\href{http://xxx.lanl.gov/abs/hep-th/9704123}{{\tt hep-th/9704123}}].

\bibitem{DVV}
R.~Dijkgraaf, E.~P. Verlinde, and H.~L. Verlinde, {\it {Matrix string theory}},
   {\em Nucl.Phys.} {\bf B500} (1997) 43--61,
  [\href{http://xxx.lanl.gov/abs/hep-th/9703030}{{\tt hep-th/9703030}}].

\bibitem{JMyers}
C.~V. Johnson and R.~C. Myers, {\it {Aspects of type IIB theory on ALE
  spaces}},  {\em Phys.Rev.} {\bf D55} (1997) 6382--6393,
  [\href{http://xxx.lanl.gov/abs/hep-th/9610140}{{\tt hep-th/9610140}}].

\bibitem{myersd}
R.~C. Myers, {\it {Dielectric branes}},  {\em JHEP} {\bf 9912} (1999) 022,
  [\href{http://xxx.lanl.gov/abs/hep-th/9910053}{{\tt hep-th/9910053}}].

\bibitem{DOT}
K.~Dasgupta, K.~Oh, and R.~Tatar, {\it {Geometric transition, large N dualities
  and MQCD dynamics}},  {\em Nucl.Phys.} {\bf B610} (2001) 331--346,
  [\href{http://xxx.lanl.gov/abs/hep-th/0105066}{{\tt hep-th/0105066}}].

\bibitem{DOT2}
K.~Dasgupta, K.~Oh, and R.~Tatar, {\it {Open / closed string dualities and
  Seiberg duality from geometric transitions in M theory}},  {\em JHEP} {\bf
  0208} (2002) 026, [\href{http://xxx.lanl.gov/abs/hep-th/0106040}{{\tt
  hep-th/0106040}}].

\bibitem{DOT3}
K.~Dasgupta, K.-h. Oh, J.~Park, and R.~Tatar, {\it {Geometric transition versus
  cascading solution}},  {\em JHEP} {\bf 0201} (2002) 031,
  [\href{http://xxx.lanl.gov/abs/hep-th/0110050}{{\tt hep-th/0110050}}].

\bibitem{ADS}
I.~Affleck, M.~Dine, and N.~Seiberg, {\it {Dynamical Supersymmetry Breaking in
  Four-Dimensions and Its Phenomenological Implications}},  {\em Nucl.Phys.}
  {\bf B256} (1985) 557.

\bibitem{ADS2}
I.~Affleck, M.~Dine, and N.~Seiberg, {\it {Dynamical Supersymmetry Breaking in
  Supersymmetric QCD}},  {\em Nucl.Phys.} {\bf B241} (1984) 493--534.

\bibitem{ADHM}
M.~Atiyah, N.~J. Hitchin, V.~Drinfeld, and Y.~Manin, {\it {Construction of
  Instantons}},  {\em Phys.Lett.} {\bf A65} (1978) 185--187.

\bibitem{MNun}
J.~M. Maldacena and C.~Nunez, {\it {Towards the large N limit of pure N=1
  superYang-Mills}},  {\em Phys.Rev.Lett.} {\bf 86} (2001) 588--591,
  [\href{http://xxx.lanl.gov/abs/hep-th/0008001}{{\tt hep-th/0008001}}].

\bibitem{KeWi}
I.~R. Klebanov and E.~Witten, {\it {Superconformal field theory on three-branes
  at a Calabi-Yau singularity}},  {\em Nucl.Phys.} {\bf B536} (1998) 199--218,
  [\href{http://xxx.lanl.gov/abs/hep-th/9807080}{{\tt hep-th/9807080}}].

\bibitem{anke3}
M.~Becker, K.~Dasgupta, S.~H. Katz, A.~Knauf, and R.~Tatar, {\it {Geometric
  transitions, flops and non-Kahler manifolds. II.}},  {\em Nucl.Phys.} {\bf
  B738} (2006) 124--183, [\href{http://xxx.lanl.gov/abs/hep-th/0511099}{{\tt
  hep-th/0511099}}].

\bibitem{LS}
R.~G. Leigh and M.~J. Strassler, {\it {Exactly marginal operators and duality
  in four-dimensional N=1 supersymmetric gauge theory}},  {\em Nucl.Phys.} {\bf
  B447} (1995) 95--136, [\href{http://xxx.lanl.gov/abs/hep-th/9503121}{{\tt
  hep-th/9503121}}].

\bibitem{tacwecht1}
F.~Benini, Y.~Tachikawa, and B.~Wecht, {\it {Sicilian gauge theories and N=1
  dualities}},  {\em JHEP} {\bf 1001} (2010) 088,
  [\href{http://xxx.lanl.gov/abs/0909.1327}{{\tt arXiv:0909.1327}}].

\bibitem{tacwecht2}
D.~Green, Z.~Komargodski, N.~Seiberg, Y.~Tachikawa, and B.~Wecht, {\it {Exactly
  Marginal Deformations and Global Symmetries}},  {\em JHEP} {\bf 1006} (2010)
  106, [\href{http://xxx.lanl.gov/abs/1005.3546}{{\tt arXiv:1005.3546}}].

\bibitem{nikulin}
V.~Nikulin, {\it {Discrete reflection groups in Lobachevsky spaces and
  algebraic surfaces}},  {\em {\it Proceedings of the international congress of
  mathematicians}, Berkeley} (1986) 654--671.

\bibitem{sengimon}
A.~Sen, {\it {A non-perturbative description of the Gimon-Polchinski
  orientifold}},  {\em Nucl. Phys.} {\bf B489} (1997) 139--159,
  [\href{http://xxx.lanl.gov/abs/hep-th/9611186}{{\tt hep-th/9611186}}].

\bibitem{sengimon2}
A.~Sen, {\it {F theory and the Gimon-Polchinski orientifold}},  {\em
  Nucl.Phys.} {\bf B498} (1997) 135--155,
  [\href{http://xxx.lanl.gov/abs/hep-th/9702061}{{\tt hep-th/9702061}}].

\bibitem{gopamu}
R.~Gopakumar and S.~Mukhi, {\it {Orbifold and orientifold compactifications of
  F - theory and M - theory to six-dimensions and four-dimensions}},  {\em
  Nucl.Phys.} {\bf B479} (1996) 260--284,
  [\href{http://xxx.lanl.gov/abs/hep-th/9607057}{{\tt hep-th/9607057}}].

\bibitem{dabholkarP}
A.~Dabholkar and J.~Park, {\it {A note on orientifolds and F-theory}},  {\em
  Phys. Lett.} {\bf B394} (1997) 302--306,
  [\href{http://xxx.lanl.gov/abs/hep-th/9607041}{{\tt hep-th/9607041}}].

\bibitem{blumZ}
J.~D. Blum and A.~Zaffaroni, {\it {An Orientifold from F theory}},  {\em
  Phys.Lett.} {\bf B387} (1996) 71--74,
  [\href{http://xxx.lanl.gov/abs/hep-th/9607019}{{\tt hep-th/9607019}}].

\bibitem{MV1}
D.~R. Morrison and C.~Vafa, {\it {Compactifications of F theory on Calabi-Yau
  threefolds. 1}},  {\em Nucl.Phys.} {\bf B473} (1996) 74--92,
  [\href{http://xxx.lanl.gov/abs/hep-th/9602114}{{\tt hep-th/9602114}}].

\bibitem{MV2}
D.~R. Morrison and C.~Vafa, {\it {Compactifications of F-Theory on Calabi--Yau
  Threefolds -- II}},  {\em Nucl. Phys.} {\bf B476} (1996) 437--469,
  [\href{http://xxx.lanl.gov/abs/hep-th/9603161}{{\tt hep-th/9603161}}].

\bibitem{ashopin}
P.~S. Aspinwall and M.~Gross, {\it {The SO(32) heterotic string on a K3
  surface}},  {\em Phys.Lett.} {\bf B387} (1996) 735--742,
  [\href{http://xxx.lanl.gov/abs/hep-th/9605131}{{\tt hep-th/9605131}}].

\bibitem{sennbps}
A.~Sen, {\it {Stable nonBPS states in string theory}},  {\em JHEP} {\bf 9806}
  (1998) 007, [\href{http://xxx.lanl.gov/abs/hep-th/9803194}{{\tt
  hep-th/9803194}}].

\bibitem{vafaT}
J.~J. Heckman, Y.~Tachikawa, C.~Vafa, and B.~Wecht, {\it {N = 1 SCFTs from
  Brane Monodromy}},  {\em JHEP} {\bf 1011} (2010) 132,
  [\href{http://xxx.lanl.gov/abs/1009.0017}{{\tt arXiv:1009.0017}}].

\bibitem{voisin}
C.~Voisin, {\it {Miroirs et involutions sur les surfaces K3}},  {\em Journées
  de Géométrie Algébrique d'Orsay} {\bf 218} (1993) 273--323.

\bibitem{borcea}
C.~Borcea, {\it {K3 surfaces with involution and mirror pairs of Calabi-Yau
  manifolds}},  {\em Essays on Mirror Manifolds II} (1997).

\bibitem{dmwit}
M.~Duff, R.~Minasian, and E.~Witten, {\it {Evidence for heterotic / heterotic
  duality}},  {\em Nucl.Phys.} {\bf B465} (1996) 413--438,
  [\href{http://xxx.lanl.gov/abs/hep-th/9601036}{{\tt hep-th/9601036}}].

\bibitem{vafaGT}
C.~Vafa, {\it {Superstrings and topological strings at large N}},  {\em
  J.Math.Phys.} {\bf 42} (2001) 2798--2817,
  [\href{http://xxx.lanl.gov/abs/hep-th/0008142}{{\tt hep-th/0008142}}].

\bibitem{katzvafa}
F.~Cachazo, B.~Fiol, K.~A. Intriligator, S.~Katz, and C.~Vafa, {\it {A
  Geometric unification of dualities}},  {\em Nucl.Phys.} {\bf B628} (2002)
  3--78, [\href{http://xxx.lanl.gov/abs/hep-th/0110028}{{\tt hep-th/0110028}}].

\bibitem{anke1}
M.~Becker, K.~Dasgupta, A.~Knauf, and R.~Tatar, {\it {Geometric transitions,
  flops and nonKahler manifolds. I.}},  {\em Nucl.Phys.} {\bf B702} (2004)
  207--268, [\href{http://xxx.lanl.gov/abs/hep-th/0403288}{{\tt
  hep-th/0403288}}].

\bibitem{anke2}
S.~Alexander, K.~Becker, M.~Becker, K.~Dasgupta, A.~Knauf, {\em et.~al.}, {\it
  {In the realm of the geometric transitions}},  {\em Nucl.Phys.} {\bf B704}
  (2005) 231--278, [\href{http://xxx.lanl.gov/abs/hep-th/0408192}{{\tt
  hep-th/0408192}}].

\bibitem{chuchai}
C.-S. Chu and D.~Giataganas, {\it {UV-divergences of Wilson Loops for
  Gauge/Gravity Duality}},  {\em JHEP} {\bf 0812} (2008) 103,
  [\href{http://xxx.lanl.gov/abs/0810.5729}{{\tt arXiv:0810.5729}}].

\bibitem{miamodel}
M.~Mia, K.~Dasgupta, C.~Gale, and S.~Jeon, {\it {Toward Large N Thermal QCD
  from Dual Gravity: The Heavy Quarkonium Potential}},  {\em Phys.Rev.} {\bf
  D82} (2010) 026004, [\href{http://xxx.lanl.gov/abs/1004.0387}{{\tt
  arXiv:1004.0387}}].

\bibitem{swncg}
N.~Seiberg and E.~Witten, {\it {String theory and noncommutative geometry}},
  {\em JHEP} {\bf 9909} (1999) 032,
  [\href{http://xxx.lanl.gov/abs/hep-th/9908142}{{\tt hep-th/9908142}}].

\bibitem{AKS}
O.~Aharony, S.~Kachru, and E.~Silverstein, {\it {New N=1 superconformal field
  theories in four-dimensions from D-brane probes}},  {\em Nucl.Phys.} {\bf
  B488} (1997) 159--176, [\href{http://xxx.lanl.gov/abs/hep-th/9610205}{{\tt
  hep-th/9610205}}].

\bibitem{vafaiqbal}
A.~Iqbal, A.~Neitzke, and C.~Vafa, {\it {A Mysterious duality}},  {\em
  Adv.Theor.Math.Phys.} {\bf 5} (2002) 769--808,
  [\href{http://xxx.lanl.gov/abs/hep-th/0111068}{{\tt hep-th/0111068}}].

\bibitem{plesser}
P.~C. Argyres, M.~R. Plesser, and A.~D. Shapere, {\it {The Coulomb phase of N=2
  supersymmetric QCD}},  {\em Phys. Rev. Lett.} {\bf 75} (1995) 1699--1702,
  [\href{http://xxx.lanl.gov/abs/hep-th/9505100}{{\tt hep-th/9505100}}].

\bibitem{dhoker2}
E.~D'Hoker, I.~Krichever, and D.~Phong, {\it {The Effective prepotential of N=2
  supersymmetric SU(N(c)) gauge theories}},  {\em Nucl.Phys.} {\bf B489} (1997)
  179--210, [\href{http://xxx.lanl.gov/abs/hep-th/9609041}{{\tt
  hep-th/9609041}}].

\bibitem{marina}
K.~Dasgupta and M.~Shmakova, {\it {On branes and oriented B fields}},  {\em
  Nucl.Phys.} {\bf B675} (2003) 205--240,
  [\href{http://xxx.lanl.gov/abs/hep-th/0306030}{{\tt hep-th/0306030}}].

\bibitem{dw}
R.~Donagi and E.~Witten, {\it {Supersymmetric Yang-Mills theory and integrable
  systems}},  {\em Nucl.Phys.} {\bf B460} (1996) 299--334,
  [\href{http://xxx.lanl.gov/abs/hep-th/9510101}{{\tt hep-th/9510101}}].

\bibitem{markman}
R.~Donagi and E.~Markman, {\it {Spectral curves, algebraically completely
  integrable Hamiltonian systems, and moduli of bundles}},
  \href{http://xxx.lanl.gov/abs/alg-geom/9507017}{{\tt alg-geom/9507017}}.

\bibitem{ArgyresFaraggiSU}
P.~C. Argyres and A.~E. Faraggi, {\it {The vacuum structure and spectrum of N=2
  supersymmetric SU(n) gauge theory}},  {\em Phys. Rev. Lett.} {\bf 74} (1995)
  3931--3934, [\href{http://xxx.lanl.gov/abs/hep-th/9411057}{{\tt
  hep-th/9411057}}].

\end{thebibliography}\endgroup

